GraphMatch: Efficient Large-Scale Graph Construction for Structure from Motion

We present GraphMatch, an approximate yet efficient method for building the matching graph for large-scale structure-from-motion (SfM) pipelines. Unlike modern SfM pipelines that use vocabulary (Voc.) trees to quickly build the matching graph and avoid a costly brute-force search of matching image pairs, GraphMatch does not require an expensive offline pre-processing phase to construct a Voc. tree. Instead, GraphMatch leverages two priors that can predict which image pairs are likely to match, thereby making the matching process for SfM much more efficient. The first is a score computed from the distance between the Fisher vectors of any two images. The second prior is based on the graph distance between vertices in the underlying matching graph. GraphMatch combines these two priors into an iterative "sample-and-propagate" scheme similar to the PatchMatch algorithm. Its sampling stage uses Fisher similarity priors to guide the search for matching image pairs, while its propagation stage explores neighbors of matched pairs to find new ones with a high image similarity score. Our experiments show that GraphMatch finds the most image pairs as compared to competing, approximate methods while at the same time being the most efficient.

==> AlgorithmOverview.tex <==
\subsection{Algorithm Overview}

The algorithm consists of two iterative main steps. The first step, 
which we call it \textit{Ranked Sampling}, attempts to find the image 
pairs that are likely to pass matching and geometric verification 
procedure. And the second step named \textit{Propagation} step, is 
for detecting the new edges given the set of discovered edges in Ranked 
Sampling step in that iteration as well as the state of the image 
graph till that iteration.

\textbf{Notation.} Table \ref{table:symbols} lists the main symbols 
we use throughout this paper. As mentioned earlier the proposed method 
takes place in an iterative manner. We use superscripts for the 
image-pair graph $\mathbf{G}$ and all the sets defined in this table 
to denote in which iteration they are. For instance, we use $\mathbf{G}^t$ 
for denoting $\mathbf{G}$ at iteration $t$. Also, for showing the 
$i^{\text{th}}$ member of each set we use subscript $i$ (\eg $I_i$.)

As mentioned before in this section, having prior information would be 
like a guidance for us and we found out that we can use Fisher 
Vectors and so our prior knowledge could be the similarity scores 
based on how much similar Fisher Vectors are. Therefore, as 
a preprocessing step and before starting our main iterative procedure, 
we initialize all the image pairs with the corresponding similarity 
scores. After the initialization, each image node $I_i$ will have a 
list of its candidates that is ranked based on the similarity scores. 

\begin{table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
Symbol & Definition and Description & Constraints\\
\hline\hline
$\mathbf{G}$ & Geometrically verified image-pair   & \\
$\mathbf{I}$ & Set of images & \\
$\mathbf{E}$ & Set of edges & \\
$\mathbf{W}$ & Set of non-edges & \\
$\mathbf{T}$ & Set of detected image triplets & \\
$V$ & Subset of image pair indices & $\mathbf{N^+}$\\
$s$ & Image-pair similarity score & $\mathbf{R}$\\
$e$ & Number of edges & $\mathbf{N^+}$\\
$\tau$ & Number of triplets & $\mathbf{N^+}$\\
$v$ & Binary variable for geometric verification & $\{0,1\}$\\
\hline
\end{tabular}
}
\caption{Symbols}
\label{table:symbols}
\end{table}


==> Discussion.tex <==
\section{Discussion}


\subsection{Comparisons to PatchMatch}

Effectively, both GraphMatch and PatchMatch~\cite{Barnes2009} are trying to do the same thing: provide a large speedup over the baseline  by effectively using propagation to ``suggest'' good potential matches. In both cases, the baseline algorithm for the respective problems faces a $O(N^2)$ computational complexity, which becomes an issue because of they each have a slow process of the inner loop.  

In our case, the inner loop involves a geometric verification test for a pair of images which requires finding corresponding SIFT features and fitting a model with RANSAC.  In the problem of patch-wise correspondences, the innerloop is the calculation of $L_2$ error between patches.  Although this distance calculation is slow enough to make the brute-force method practically unfeasible for large images (thereby requiring acceleration by PatchMatch), we note that the inner loop of our problem is much more complex and computationally expensive.  

Therefore, although the baseline methods for both problems are $O(N^2)$, the constants are significantly bigger in our case.  This means that the time savings from GraphMatch are bigger than that of PatchMatch, and indeed we see that in our results XXXXXX.


==> OLD_PropagationStep.tex <==
\subsection{Propagation Step}
After step 1, a set of new edges have been discovered, and accordingly a 
set of image nodes $\mathbf{I}$ in the graph now have found some new 
adjacents. Propagation step aims at detecting new edges given the set of 
discovered edges in the Ranked Sampling step $V^t$ at iteration $t$ and 
the graph $\mathbf{G}^{t-1}$. 

We assume if two image nodes are connected then each one of them are 
likely to be connected to the other node's connections. Hence, we came up
with this idea that we can get all the edges, \ie all the image pairs that 
have successfully passed geometric verification, and then we attempt to 
propagate this connectivity by performing the geometric verification on 
a selection of the connections of connections of the each image nodes. 
Clearly, the selection is constrained on picking the ones that have not 
been yet verified.


Let's consider the case where edges are extracted from a set of image 
triplets $T^t = T(\mathbf{E}^t, \mathbf{G}^{t-1})$. A triplet is defined 
as follows: if two edges defined by $A - B$ and $B 
- C$, then $A - C$ is likely to be an edge. 
The goal in propagation is to select $\tau$ image triplets that like to 
generate new edges. This can be described mathematically as follows:

\begin{equation}
    \label{eq:3}
    \small
    \underset{V}{max} \mathbf{E} [e^t|T^t, s_T]=
    \sum_{e=1}^{\tau}{{\tau}\choose{e}} \prod_{i\in V(\tau), i=1}^{e}
    \text{Pr}(v_i=1|d_i)
\end{equation}

where $i\in V(T)$ is the subset of image pair indices in the set of
discovered triplets $T$. 

[POINT HERE IS TO TALK ABOUT OUR PROPOSED WAYS TO SELECT THE TOP $\tau$ TRIPLETS IN ORDER TO EXECUTE PROPAGATION)

We came up with this idea that we have 4 ways to select the top $\tau$ image triplets out of all the triplets we have. Suppose we have an image triplet $A - B - C$ and the two verified image pairs that we have in this triplet are $A - B$ and $B - C$. 

[SPEAKING OF INLIER RATIO SCORE] We get the number of inlier features between the two image pairs $A - B$ and $B - C$, as $M_{AB}$ and $M_{BC}$ and compute the ratio of each to the minimum of the two numbers of features for each image. For instance, for image pair $A - B$ we would have $F_A$ and $F_B$ which indicate the number of features that image $A$ and $B$ have, respectively. We compute the ratio of inliers $M_{AB}$ to the minimum of $F_A$ and $F_B$. We repeat this calculation for the image pair $B - C$ as well. We observed that the number that we get by multiplying these two inlier ratios would give us a 


==> OLD_ProposedMethod.tex <==
\section{Proposed Algorithm: GraphMatch}

Our proposed algorithm, GraphMatch, is inspired by the PatchMatch algorithm and also has two main stages: sampling and propagation.  The 






THIS IS THE STUFF WRITTEN EARLIER BY ATIEH






Our main approach to the problem is designing an algorithm for finding 
the interconnectivity of the image graph. The approach we take may not 
be the only possible way to solve the matching problem, however it 
meets our goal which is connecting the images so that in next stage in
SfM pipeline it gives us the complete models with descent quality.

Now suppose that we are given a set of images, $\mathbf{I} = 
\{I_1, I_2, \ldots, I_n\}$ as input, and the task for us is to detect
the connections between images as quickly as possible and that
is achievable if could intelligently perform matching and geometric 
verification procedure on images, \ie not going through all the image
pairs but only the ones that by a good probability would be our true 
guesses. 

The image graph $G$ eventually will be filled with detected edges in 
which the nodes are considered to be the given images, and the edges 
between each pair of nodes indicate that the corresponding nodes could 
successfully pass the geometric verification.

This section presents a ranked method for finding the edges of the graph.
The algorithm works by searching in the space of image pairs and every 
time picking the pairs that have this potential to be the new edges in 
the image graph $G$.    

We utilize a prior information to figure out the adjacency likelihood of 
the image pairs. We assume those image pairs that have more visual 
similarity would be good choices for performing geometric verification 
on. So for that, after experimenting with different kinds of global 
descriptors we arrived to this conclusion that computing Fisher 
descriptor for each image would be the best option, as it discovers 
more edges in the same amount of time compared to using other global 
descriptors.

After that for every image pair we compute the distance between their 
descriptors. The less distance the image pairs have, it shows that the 
more visual similarity they would have, and so the higher rank they 
would get to be selected. In order to calculate the similarity score 
for each image-pair we use Euclidean distance as our image similarity 
metric.




%------------------------------------------------------------------------
\input{AlgorithmOverview.tex}

%-------------------------------------------------------------------------
\input{RankedSamplingStep.tex}

%-------------------------------------------------------------------------
\input{PropagationStep.tex}

%-------------------------------------------------------------------------
\subsection{Combining Steps}

%-------------------------------------------------------------------------
\input{TerminationCriterion.tex}

==> OLD_TerminationCriterion.tex <==
\subsection{Termination Criterion}
The naive approach of this algorithm is that it executes until no further 
potential edges left that we can do the geometric verification procedure 
on it. However, there would not be any improvement over brute-force 
method with this approach. We found out the algorithm works well if we set 
a maximum for the number of adjecents that an image node can have. This 
way we only continue doing sampling and propagation on those image nodes 
that have less than a certain number of adjacents.


==> RankedSamplingStep.tex <==
\subsection{Ranked Sampling Step}

In ranked sampling step, at each iteration, we get the set of all the 
image nodes $\mathbf{I}$ and for each node we sample from the remaining 
nodes the ones that have the highest rank in the ranked candidate list 
corresponding to sampler node. This way we will have a set of image pairs
that we can perform geometric verification procedure on them. So, our goal 
here in this step is to select a certain number of image pairs "$k$", 
that maximizes the expected number of edges from the selection conditioned 
on selecting pairs that have not been yet verified. With the assumption 
that the algorithm is running at iteration $t$, this objective can be
written as follows:

\begin{equation}
    \label{eq:1}
    \underset{V}{\max} \mathbf{E}[e^t|s_V] = \sum_{e=1}^{k}e
    \text{Pr}(e^t=e|s_V,\mathbf{G}^{t-1})
\end{equation}
where $\text{Pr}(e^t=e|s_V,G^{(t-1)})$ is the probability of getting $e$ 
number of edges given the image-pair similarity scores $s_V$ of the subset
$V$, and the graph $G^{t-1}$ at iteration $t-1$. The aforementioned 
probability is calculated as follows:

\begin{equation}
    \label{eq:2}
    \small
    \text{Pr}(e^t=e|s_V,G^{(t-1)})
    = {{k}\choose{e}}\prod_{i=1}^{e}\text{Pr}(v_i=1|d_i,G^{t-1})
\end{equation}
where $\text{Pr}(v_i=1|d_i)$ is the probability of $i^\text{th}$ image pair 
passing geometric verification (\ie $v_i=1$) given that we know the image 
pair similarity score $s_i$.


==> TerminationCriterion.tex <==
\subsection{Termination Criterion}
\label{sec:TerminationCriterion}
